Compositional Specifications for ioco Testing

Model-based testing is a promising technology for black-box software and hardware testing, in which test cases are generated automatically from high-level specifications. Nowadays, systems typically consist of multiple interacting components and, due to their complexity, testing presents a considerable portion of the effort and cost in the design process. Exploiting the compositional structure of system specifications can considerably reduce the effort in model-based testing. Moreover, inferring properties about the system from testing its individual components allows the designer to reduce the amount of integration testing. In this paper, we study compositional properties of the IOCO-testing theory. We propose a new approach to composition and hiding operations, inspired by contract-based design and interface theories. These operations preserve behaviors that are compatible under composition and hiding, and prune away incompatible ones. The resulting specification characterizes the input sequences for which the unit testing of components is sufficient to infer the correctness of component integration without the need for further tests. We provide a methodology that uses these results to minimize integration testing effort, but also to detect potential weaknesses in specifications. While we focus on asynchronous models and the IOCO conformance relation, the resulting methodology can be applied to a broader class of systems.

==> proofs.tex <==
\onecolumn

\section{Proofs}
\label{sec:proofs}

\setcounter{lemma}{0}
\setcounter{theorem}{2}
\setcounter{proposition}{0}


\begin{lemma}
\label{lemma:exits_lcl_env}
For any two compatible $\iolts$ $A$ and $B$ there exists a maximal composition-friendly environment for $A \parallel B$.
\end{lemma}
\begin{IEEEproof}
Consider compatible $\iolts$ $A$ and $B$.
By definition $A \parallel B$ have at least one friendly environment.
Suppose that there is no maximal composition-friendly environment for $A \parallel B$.
This implies that there are two  composition-friendly environments, say $E_1$ and $E_2$, such that every composition-friendly environment $E$ satisfies:
\begin{equation} \label{eq:egle_0}
  \traces{E} \not\supseteq \traces{E_1} \cup \traces{E_2}.
\end{equation}
W.l.o.g.\ assume that $E_1$ and $E_2$ have pairwise disjoint sets of states, except for their initial state, which is the same.
We construct the $\iolts$ $E_{lc} = (Q_{lc}, \InputLabels, \OutputLabels, T_{lc}, \qinit_{lc})$, s.t.\
\begin{itemize}
\item $Q_{lc} \;=\  Q_{E_1} \cup Q_{E_2}$,
\item $T_{lc} \;=\; T_{E_1} \cup T_{E_2}$,
\item $\qinit_{lc} \;=\; \qinit_{E_1} \;=\; \qinit_{E_2}$.
\end{itemize}
$E_{lc}$ starts in the shared initial state and then behaves likes $E_1$ or $E_2$, so $\traces{E} = \traces{E_1} \cup \traces{E_2}$.

Suppose that $E_{lc}$ is not a composition friendly environment for $A\parallel B$.
This means that there exists a state $s=((q_A, q_B), q_E)$ reachable in $(A\parallel B)\parallel E_{lc}$, such that $s$ is ambiguous in $(A \parallel B) \parallel E$ or $(q_A, q_B)$ is ambiguous in $A \parallel B$.
State $s$ is also reachable in  $(A\parallel B)\parallel E_1$ or $(A\parallel B)\parallel E_2$, hence either $E_1$ or $E_2$ would not be a composition-friendly environment for $A \parallel B$.
By contradiction, $E_{lc}$ is a friendly environment for $A \parallel B$.

We conclude that $E_{lc}$ is a composition-friendly environment for $A \parallel B$. It violates assumption \eqref{eq:egle_0}, so by contradiction there exists a maximal friendly environment for $A \parallel B$.
\end{IEEEproof}

\bigskip

% \begin{lemma}
% \label{lemma:int_comp_prop}
% Let $A,B,C$ be $\iolts$ that are mutually compatible.
% Then the following statements are valid:
% \begin{enumerate}
%   \item $\straces{\intcomp{A}{B}}$ is uniquely defined,
%   \item $\straces{A  \otimes B} \;=\; \straces{B \otimes A}$,
%   \item $\straces{({\intcomp{A}{B}}) \otimes C} \;=\; \straces{A \otimes (B \otimes C)}$,
%   \item $\straces{\intcomp{A}{B}} \subseteq \straces{A \parallel B}$,
%   \item $\text{if $A$ and $B$ are receptive, then }\straces{A\otimes B} = \straces{A \parallel B}$.
% \end{enumerate}
% \end{lemma}
% \begin{IEEEproof}
% TODO.
% \end{IEEEproof}

% \bigskip

\begin{lemma}
  The following two statements hold:
  \begin{enumerate}
  \item For any two $\riolts$ $A$ and $B$, $\straces{\intcomp{A}{B}} = \straces{A \parallel B}$. 
  \item For a $\riolts$ $A$ and $\Sigma \subseteq \OutputLabels_A$ we have $\straces{\fhide{A}{\Sigma}} = \straces{\hide{A}{\Sigma}}$
  \end{enumerate}
\end{lemma}
\begin{IEEEproof}
First we prove an auxiliary result. Let $A$ be an $\riolts$, $E$ be its maximal friendly environment and $A_E$ be the $E$-reachable fragment of $A$. By  definition environment $E$ accepts all outputs issued by $A$. Moreover, since $A$ is receptive and $E$ is maximal, every state of the environment provides all inputs to $A$. As a consequence, $E$ does not restrict $A$, so $\straces{A_E} = \straces{A}$.

We prove statement 1). The parallel composition $A \parallel B$ is also an $\riolts$. $A$ and $B$ are receptive, so there are no ambiguous states in $A \parallel B$. As a consequence, the maximal friendly environment $E$ of $A\parallel B$ is also a composition-friendly environment $E$ of $A \parallel B$. The friendly composition $\intcomp{A}{B}$ is the $E$-reachable fragment of $A \parallel B$, so by our auxiliary result $\straces{\intcomp{A}{B}} = \straces{A \parallel B}$.

Now we prove statement 2). Since $A$ is a receptive module, then so is $\hide{A}{\Sigma}$. Let $E$ be a maximal friendly environment for $\hide{A}{\Sigma}$. The friendly composition $\fhide{A}{\Sigma}$ is the $E$-reachable fragment of $\hide{A}{\Sigma}$, so by our auxiliary result $\straces{\fhide{A}{\Sigma}} = \straces{\hide{A}{\Sigma}}$.
\end{IEEEproof}


\bigskip

\begin{lemma}
\label{lemma:projection_1}
Let $A$ and $B$ be two compatible $\iolts$.
Then
\begin{align*}
&\forall \sigma \in \straces{\intcomp{A}{B}}: \\
&\quad ((q_A, q_B), q_E) \in \intcomp{A}{B} \;\after\; \sigma \implies\\
&\quad (q_A \in A \;\after\; \projection{\sigma}{\Labels_A\cup \{\delta\}} \land q_B \in B \;\after\; \projection{\sigma}{\Labels_B\cup \{\delta\}}).
\end{align*}
\end{lemma}
\begin{IEEEproof}
Proof is by induction on the length of $\sigma$. 

% TODO explain more
For $\sigma=\epsilon$ the property holds, because by definition $((\qinit_A, \qinit_B), \qinit_E)$ is the initial state of $\intcomp{A}{B}$ and any transition 
$((\qinit_A, \qinit_B), \qinit_E) \xRightarrow{\epsilon}_{\susp{\intcomp{A}{B}}} ((q_A, q_B), q_E)$ can be matched by transitions
\[\qinit_A \xRightarrow{\epsilon}_\susp{A} q_A \qquad \qinit_A \xRightarrow{\epsilon}_\susp{B} q_B.\]

Assume that the property holds for trace $\sigma$ and suppose that 
\[((q_A, q_B), q_E) \in \intcomp{A}{B} \;\after\; \sigma \alpha.\]
Then there exists a predecessor state  $((q'_A, q'_B), q'_E) \in \intcomp{A}{B} \;\after\; \sigma$ s.t. 
\[((q'_A, q'_B), q'_E) \xrightarrow{\alpha}_{\susp{\intcomp{A}{B}}} ((q^\star_A, q^\star_B), q^\star_E) \xRightarrow{\epsilon}_{\susp{\intcomp{A}{B}}} ((q_A, q_B), q_E)\]
By the induction hypothesis 
\[q'_A \in A \;\after\; \projection{\sigma}{\Labels_A\cup \{\delta\}} \quad q'_B \in B \;\after\; \projection{\sigma}{\Labels_B\cup \{\delta\}}.\]

We consider different cases for $\alpha$.
Suppose that $\alpha$ is local to $A$, i.e. $\alpha \in \Labels_A\setminus \Labels_B$. 
Then the transitions 
\[q'_A \xrightarrow{\alpha}_\susp{A} q^\star_A \xRightarrow{\epsilon}_\susp{A} q_A\] is possible by the definition of friendly composition, which gives $ q_A \in A \;\after\; \projection{\sigma\alpha}{\Labels_A\cup \{\delta\}}$ as required.
From the observations
\[\projection{\sigma\alpha}{\Labels_B\cup \{\delta\}} = \projection{\sigma}{\Labels_B\cup \{\delta\}}\qquad q'_B=q^\star_B \qquad q^\star_B \xRightarrow{\epsilon}_\susp{B} q_B\]
we get
$q_B \in B\;\after\;\projection{\sigma\alpha}{\Labels_B\cup \{\delta\}}$
so the property holds. The argument for $\alpha \in \Labels_B\setminus \Labels_A$ is symmetric.

Suppose that $\alpha \in \Labels_A\cap \Labels_B$.
Then transitions 
\[q'_A \xrightarrow{\alpha}_\susp{A} q^\star_A \xRightarrow{\epsilon}_\susp{A} q_A\qquad q'_B \xrightarrow{\alpha}_\susp{B} q^\star_B \xRightarrow{\epsilon}_\susp{B} q_B\] 
are possible, so the lemma holds.

Let $\alpha = \delta$. 
We show that $q'_A, q'_B$ are quiescent in $A$ and $B$, respectively.
Suppose that $q'_A$ is not quiescent in $A$. If $q'_A$ had an outgoing $\tau$-transition, then state $((q'_A, q'_B), q'_E)$ would also have a $\tau$-transition in $\intcomp{A}{B}$, which contradictions that assumption that $((q'_A, q'_B), q'_E)$ is quiescent. 
Similarly, if $q'_A$ had some output action, then by definition of a friendly environment  state $((q'_A, q'_B), q'_E)$ would also have this action, so it would not be quiescent.
By contradiction $q'_A$ is quiescent in $A$ and the same argument shows that $q'_B$ is quiescent in $B$. 
This implies that the following transitions are possible
\[q'_A \xrightarrow{\delta}_\susp{A} q'_A = q_A\qquad q'_B \xrightarrow{\delta}_\susp{B} q'_B = q_B\] 
so the lemma holds.

\end{IEEEproof}

\bigskip

\begin{lemma}
\label{lemma:projection_2}
Let $A$ and $B$ be two compatible $\iolts$.
Then
\begin{align*}
&\forall  \sigma\in \straces{\intcomp{A}{B}}:   \\
&\qquad(q_A \in A \;\after\; \projection{\sigma}{\Labels_A\cup \{\delta\}} \land q_B \in B \;\after\; \projection{\sigma}{\Labels_B\cup \{\delta\}}) \implies\\
&\qquad\exists q_E\in Q_E: ((q_A, q_B), q_E) \in \intcomp{A}{B} \;\after\; \sigma.
\end{align*}
where $E$ is the friendly environment used in construction of $\intcomp{A}{B}$.
\end{lemma}
\begin{IEEEproof}
We first prove an auxiliary lemma. Let $A$ and $B$ be two compatible $\iolts$ and $\sigma$ be an s-trace in $\intcomp{A}{B}$.
Then
\begin{align*}\label{eq:projection_2}
&\forall (\cdot, q_E) \in \intcomp{A}{B} \;\after\; \sigma:   \\
&\qquad(q_A \in A \;\after\; \projection{\sigma}{\Labels_A\cup \{\delta\}} \land q_B \in B \;\after\; \projection{\sigma}{\Labels_B\cup \{\delta\}}) \implies\\
&\qquad((q_A, q_B), q_E) \in \intcomp{A}{B} \;\after\; \sigma.  
\end{align*}
where $E$ is the friendly environment used in construction of $\intcomp{A}{B}$.

Assume that the auxiliary lemma holds.
If $\sigma\in \straces{\intcomp{A}{B}}$, then there exists some $(\cdot, q_E) \in \intcomp{A}{B} \;\after\; \sigma$. Lemma \ref{lemma:projection_2} follows from the auxiliary lemma.

Proof of the auxiliary lemma is by induction on the length of $\sigma$. 
For the induction base let $\sigma = \epsilon$. Assume that $((s_A, s_B), q_E) \in \intcomp{A}{B} \;\after\; \epsilon$.
This means that $\intcomp{A}{B}$ has a transition
\[((\qinit_A, \qinit_B), \qinit_E) \xRightarrow{\epsilon}_{\susp{\intcomp{A}{B}}} ((s_A, s_B), q_E).\]
$\tau$-transitions in $\intcomp{A}{B}$ arise from independent $\tau$-transitions in $A, B$ and $E$, so
$\qinit_E \xRightarrow{\epsilon}_{E} q_E$.
Let  $q_A \in A \;\after\; \epsilon$ and $q_B \in B\;\after\; \epsilon$. 
Then by definition of friendly composition
$((\qinit_A, \qinit_B), \qinit_E) \xRightarrow{\epsilon}_{\susp{\intcomp{A}{B}}} ((q_A, q_B), q_E)$. 

For the induction step assume that the property holds for trace $\sigma$.
Consider arbitrary 
\[((s_A, s_B), q_E) \in \intcomp{A}{B} \;\after\; \sigma\alpha\]
and assume that
\[ q_A \in A \;\after\; \projection{\sigma\alpha}{\Labels_A\cup \{\delta\}} \qquad q_B \in B \;\after\; \projection{\sigma\alpha}{\Labels_B\cup \{\delta\}}.\]
State $((s_A, s_B), q_E)$ has a predecessor state $((s'_A, s'_B), q'_E) \in \intcomp{A}{B}\;\after\; \sigma$ s.t.:
\begin{equation} \label{eq:projection_2_0}
((s'_A, s'_B), q'_E) \xrightarrow{\alpha}_\susp{\intcomp{A}{B}} ((s^\star_A, s^\star_B), q^\star_E) \xRightarrow{\epsilon}_\susp{\intcomp{A}{B}} ((s_A, s_B), q_E).  
\end{equation}

We consider possible cases for $\alpha$.
Let $\alpha \in \Labels_A \setminus \Labels_B$. 
There exists a predecessors $q'_A$ of $q_A$:
\begin{equation}  \label{eq:projection_2_7}
  q'_A \in A\;\after\; \projection{\sigma}{\Labels_A \cup \{\delta\}} \quad \text{s.t.}\quad q'_A \xrightarrow{\alpha}_\susp{A} q^\star_A \xRightarrow{\epsilon}_\susp{A} q_A.
\end{equation}
From $\projection{\sigma\alpha}{\Labels_B \cup \{\delta\}}=\projection{\sigma}{\Labels_B \cup \{\delta\}}$ it follows that $q_B \in B\;\after\; \projection{\sigma}{\Labels_B \cup \{\delta\}}$. Then, by the induction hypothesis:
\[ \forall (\cdot, q) \in \intcomp{A}{B}\;\after\; \sigma: ((q'_A, q_B), q) \in \intcomp{A}{B} \;\after\; \sigma.\]
Instantiating $q$ with $q'_E$ gives
\[ ((q'_A, q_B), q'_E) \in \intcomp{A}{B} \;\after\; \sigma.\]
From \eqref{eq:projection_2_0} and the definition of friendly composition we get:
\begin{equation}\label{eq:projection_2_1}
q'_E \xrightarrow{\alpha}_E q^\star_E \xRightarrow{\epsilon}_E q_E.
\end{equation}
By \eqref{eq:projection_2_7}, \eqref{eq:projection_2_1} and the definition of friendly composition state $((q'_A, q_B), q'_E)$ can execute action $\alpha$ in $\intcomp{A}{B}$ and then any following silent transitions that lead to $((q_A, q_B), q_E)$:
\[ ((q'_A, q_B), q'_E) \xrightarrow{\alpha}_{\susp{\intcomp{A}{B}}} (q^\star_A, q_B, q^\star_E) \xRightarrow{\epsilon}_{\susp{\intcomp{A}{B}}} ((q_A, q_B), q_E).\]
This gives $((q_A, q_B), q_E) \in \intcomp{A}{B} \;\after\; \sigma\alpha$ as required. 
Symmetrical argument holds for $\alpha \in \Labels_B\setminus \Labels_A$.

Let $\alpha \in \Labels_A \cap \Labels_B$. 
States $q_A$ and  $q_B$ have some predecessors $q'_A, q'_B$:
\begin{align}
q'_A \in A\;\after\; \projection{\sigma}{\Labels_A \cup \{\delta\}} \quad \text{s.t.}\quad q'_A \xrightarrow{\alpha}_\susp{A} q^\star_A \xRightarrow{\epsilon}_\susp{A} q_A.\label{eq:projection_2_2}\\ 
q'_B \in B\;\after\; \projection{\sigma}{\Labels_B \cup \{\delta\}} \quad \text{s.t.}\quad q'_B \xrightarrow{\alpha}_\susp{B} q^\star_B \xRightarrow{\epsilon}_\susp{B} q_B.\label{eq:projection_2_3}
\end{align}
It follows from \eqref{eq:projection_2_0} that
\begin{equation}  \label{eq:projection_2_5}
 q'_E \xrightarrow{\alpha}_E q^\star_E \xRightarrow{\epsilon}_E q_E.
\end{equation}
Then by the induction hypothesis we get:
\[((q'_A, q'_B), q'_E) \in \intcomp{A}{B} \;\after\; \sigma.\]
By \eqref{eq:projection_2_5}, \eqref{eq:projection_2_2}, \eqref{eq:projection_2_3} and the definition of friendly composition  the following transition is possible in $\intcomp{A}{B}$:
\[ ((q'_A, q'_B), q'_E) \xrightarrow{\alpha}_{\susp{\intcomp{A}{B}}} ((q^\star_A, q^\star_\susp{B}), q^\star_E) \xRightarrow{\epsilon}_{\susp{\intcomp{A}{B}}} ((q_A, q_B), q_E).\]

Let $\alpha = \delta$. 
We note that in \eqref{eq:projection_2_0} $q'_E = q^\star_E = q_E$.
State $q_E$ cannot not have any outgoing $\tau$-transitions, because otherwise $((q'_A, q'_B), q'_E)$ would not be quiescent.
States $q_A, q_B$ are quiescent, therefore:
\begin{align*}
q_A \in A\;\after\; \projection{\sigma}{\Labels_A \cup \{\delta\}} \quad \text{and}\quad q_A \xrightarrow{\delta}_\susp{A} q_A.\\
q_B \in B\;\after\; \projection{\sigma}{\Labels_B \cup \{\delta\}} \quad \text{and}\quad q_B \xrightarrow{\delta}_\susp{B} q_B.
\end{align*}
By the induction hypothesis
\[((q_A, q_B), q'_E) \in \intcomp{A}{B} \;\after\; \sigma.\]
State  $((q_A, q_B), q'_E)$ cannot have any $\tau$-transitions, because $q_A, q_B$ are quiescent and $q_E$ does not have such transitions.
Any output transitions in $\intcomp{A}{B}$ arise from synchronization of $A$ or $B$ with the friendly environment. States $q_A, q_B$ are quiescent, hence $((q_A, q_B), q_E)$ does have any output actions. 
It follows that $((q_A, q_B), q_E)$ is quiescent in $\intcomp{A}{B}$:
\[ (q_A, q_B, q_E) \xrightarrow{\delta}_{\susp{\intcomp{A}{B}}} ((q_A, q_B), q_E).\]
Since $((s_A, s_B), q_E)$ was arbitrary, so the auxiliary lemma holds for any $((s_A, s_B), q_E) \in \intcomp{A}{B} \;\after\; \sigma\alpha.$
\end{IEEEproof}

\bigskip



\begin{theorem}
\label{th:ioco_comp}
Given two compatible $\riolts$ $I_1$ and $I_2$ and two compatible $\iolts$ $S_1$ and $S_2$, we have
\[
I_1 \; \ioco \; S_1 \wedge I_2 \; \ioco \; S_2 \rightarrow (\intcomp{I_1}{I_2}) \; \ioco \; (\intcomp{S_1}{S_2}).\]
\end{theorem}
\begin{IEEEproof}
Let $E_S, E_I$ be the friendly environments used in construction of $\intcomp{S_1}{S_2}$ and $\intcomp{I_1}{I_2}$, respectively.
Assume that $I_1 \; \ioco \; S_1$ and $I_2 \; \ioco \; S_2$. 
Let $\sigma$ be an arbitrary suspension trace in  $\intcomp{S_1}{S_2}$
and let 
\[ P = \intcomp{S_1}{S_2} \; \after_{S_1\otimes S_2} \; \sigma \qquad R = \intcomp{I_1}{I_2} \; \after_{\intcomp{I_1}{I_2}} \; \sigma.\]
Suppose that $\alpha \in \out{R}{\intcomp{I_1}{I_2}}$. 
We need to show that $\alpha \in \out{P}{\intcomp{S_1}{S_2}}.$

Consider an arbitrary state  $((q_{I_1},q_{I_2}),q_{E}) \in R$ such that 
\[\alpha \in \out{((q_{I_1}, q_{I_2}), q_{E})}{\intcomp{I_1}{I_2}}.\]
Consider different cases for $\alpha$.

Let$\alpha \in \OutputLabels_1 \backslash \InputLabels_2$.
By Lemma~\ref{lemma:projection_1}, we have that 
\[q_{I_1} \in I_1 \; \after_{I_1} \projection{\sigma}{\Labels_1\cup\{\delta\}}\qquad\projection{\sigma}{\Labels_1\cup\{\delta\}}\in \straces{S_1}.\]
By the definition of friendly composition $\alpha \in \out{q_{I_1}}{I_1}$.
S-trace $\projection{\sigma}{\Labels_1\cup\{\delta\}}$ is shared between $S_1$ and $I_1$, so from the assumption  $I_1 \; \ioco \; S_1$ it follows that:
 \[\alpha \in \out{S_1 \; \after \; \projection{\sigma}{\Labels_1\cup\{\delta\}}}{},\]
so there exists a state 
\[q_{S_1} \in S_1 \;\after\; \projection{\sigma}{\Labels_1\cup\{\delta\}}{}\]
s.t. $\alpha \in \out{q_{S_1}}{S_1}$.
By Lemma~\ref{lemma:projection_1}, there exists a state
\[q_{S_2} \in S_2 \;\after\; \projection{\sigma}{\Labels_2\cup\{\delta\}}.\]
Then by Lemma~\ref{lemma:projection_2}
\[\exists q_E\in Q_{E_S}: ((q_{S_1}, q_{S_2}), q_E) \in \intcomp{S_1}{S_2} \;\after\; \sigma.\]
In composition $S_1 \parallel S_2$ state $(q_{S_1}, q_{S_2})$ has an outgoing action $\alpha$. 
Friendly environment $E$ must accept on $\alpha$, so $\alpha \in \out{((q_{S_1}, q_{S_2}), q_E)}{\intcomp{A}{B}}$ as required.

Let $\alpha \in \OutputLabels_2 \backslash \InputLabels_1$. The proof is symmetric to the previous case.

Let $\alpha \in \OutputLabels_1 \wedge \alpha \in \InputLabels_2$.
Following the same argument as in the first case, we get
\[\exists q_E\in Q_{E_S}: ((q_{S_1}, q_{S_2}), q_E) \in \intcomp{S_1}{S_2} \;\after\; \sigma.\]
s.t.  $\alpha \in \out{S_1 \; \after \; \projection{\sigma}{\Labels_1\cup\{\delta\}}}{}$.
In $S_1 \parallel S_2$ state $q_{S_2}$ must accept  $\alpha$, because otherwise $((q_{S_1}, q_{S_2}), q_E)$ would be an ambiguous state in $S_1 \parallel S_2$ and $E$ would not be a friendly environment. By definition of a friendly environment $E$ must synchronize on $\alpha$, so $\alpha \in \out{((q_{S_1}, q_{S_2}), q_E)}{\intcomp{A}{B}}$.

Let $\alpha \in \OutputLabels_2 \wedge \alpha \in \InputLabels_1$. The proof is symmetric to the previous case.

Let $\alpha=\delta$.
We note that state $((q_{I_1}, q_{I_2}), q_E)$ is quiescent $\intcomp{I_1}{I_2}$.
We show that $q_{I_1}, q_{I_2}$ are quiescent in $I_1$ and $I_2$. 
If $q_{I_1}$ or $q_{I_2}$ had an output transition, then $((q_{I_1}, q_{I_2}), q_E)$ would also have this action by definition of a friendly environment; but then $((q_{I_1}, q_{I_2}), q_E)$ would not be quiescent.
Similarly, if $q_{I_1}$ or $q_{I_2}$ had a $\tau$-transition, then state $((q_{I_1}, q_{I_2}), q_E)$ would also have $\tau$-transition and would not be quiescent.
By contradiction $q_{I_1}$ and $q_{I_2}$ are quiescent, so
\[ \delta \in \out{q_{I_1}}{I_1} \qquad \delta \in \out{q_{I_2}}{I_2}.\]
By Lemma \ref{lemma:projection_1} and assumption $I_i \;\ioco\; S_i, i=1,2$ we get
\[ \delta \in \out{S_1 \;\after\; \projection{\sigma}{\Labels_1\cup\{\delta\}}}{} \qquad \delta \in \out{S_1 \;\after\; \projection{\sigma}{\Labels_1\cup\{\delta\}}}{}.\]
This implies that there are states $q_{S_1}, q_{S_2}$:
\begin{align*}
  q_{S_1} \in S_1 \;\after\; \projection{\sigma}{\Labels_1\cup\{\delta\}} \quad\text{s.t.}\quad \delta\in \out{q_{S_1}}{S_1}\\
  q_{S_2} \in S_2 \;\after\; \projection{\sigma}{\Labels_2\cup\{\delta\}} \quad\text{s.t.}\quad \delta\in \out{q_{S_2}}{S_2}
\end{align*}
From Lemma \ref{lemma:projection_2} we obtain
\[ \exists q_E\in Q_{E_S}: ((q_{S_1}, q_{S_2}), q_E) \in \intcomp{S_1}{S_2}\;\after\; \sigma. \]
Transition systems are allowed to make only finite number of $\tau$-transitions from a given state. So there exists $q'_E$ reachable by $\tau$-transitions from $q_E$  in $E_S$, s.t. $q'_E$ does not have any $\tau$-transitions:
\[ q_E \xRightarrow{\epsilon}_{E_S} q'_E \quad\text{s.t.}\quad q_E \not \xrightarrow{\tau}_{E_S}. \]
State $((q_{S_1}, q_{S_2}), q'_E)$ is also reachable by suspension trace $\sigma$ in $\intcomp{S_1}{S_2}$.
This state cannot have any $\tau$-transitions, because none of $q_{S_1}, q_{S_2}$ or $q'_E$ has them.
Moreover, $((q_{S_1}, q_{S_2}), q'_E)$ does not have any output actions, because $q_{S_1}, q_{S_2}$ are quiescent and the friendly environment by itself does not generate output actions in $\intcomp{S_1}{S_2}$.
We conclude that $((q_{S_1}, q_{S_2}), q'_E)$ is quiescent in $\intcomp{S_1}{S_2}$, so 
\[ \delta \in \out{((q_{S_1}, q_{S_2}), q'_E)}{\intcomp{S_1}{S_2}}\] 
and the theorem holds.
\end{IEEEproof} 

\bigskip
\begin{lemma}
\label{lemma:outdelta}
Given  an $\iolts$ $A$ and its friendly environment $E$, it holds that
\[ \forall \sigma \in \straces{A_E}, \forall \alpha \in \OutputLabels_A \cup \{\delta\}:  \sigma\alpha \in \straces{A} \implies \sigma\alpha \in \straces{A_E},\]
where $A_E$ is the $E$-reachable fragment of $A$.
\end{lemma}
\begin{IEEEproof}
Assume that $\sigma  \in \straces{A_E}$ and $\sigma\alpha \in \straces{A}$.
Then, there is a state $(q_A, q_E) \in A_E \;\after\; \sigma$ s.t. $q_A \,\xrightarrow{\alpha}_{A_\delta}\, q'_A$.

Let $\alpha \in \OutputLabels_A$. 
By definition of a friendly environment, state $q_E$ must  accept $\alpha$:
\[ \exists q'_E\in Q_E: \;q_E \,\xrightarrow{\alpha}_E\, q'_E. \]
Then, by definition of friendly composition the following transition is possible in $A_E$:
\[ (q_A, q_E) \,\xrightarrow{\alpha}_\susp{A_E} \, (q'_A, q'_E), \]
so $\sigma\alpha \in \straces{A_E}$.

Let $\alpha = \delta$. Then state $q_A$ is quiescent in $A$.
By definition a friendly environment,  make only a finite number of $\tau$-transitions, so $q_E$ can reach by $\tau$-transitions a state $q'_E$ that has no $\tau$-transitions available:
\[ q_E \,\xRightarrow{\epsilon}_E\, q'_E \qquad q'_E\not \xrightarrow{\tau}_E.\]
Then, state $(q_A, q_E)$ can reach $(q_A, q'_E)$ by $\tau$-transitions in $A_E$:
\[ (q_A, q_E)\,\xRightarrow{\epsilon}_\susp{A_E}\, (q_A, q'_E). \]
State $(q_A, q'_E)$ does not have any output actions, since $q_A$ is quiescent and the friendly environment by itself cannot add output actions to $A_E$. 
State $(q_A, q'_E)$ also does not have any $\tau$-transitions, because neither of $q_A$ or $q'_E$ has them. 
This implies that $(q_A, q'_E)$ is quiescent and the following transitions are possible in $A_E$:
\[ (q_A, q_E)\,\xRightarrow{\epsilon}_\susp{A_E}\, (q_A, q'_E)\, \xrightarrow{\delta}_\susp{A_E} (q_A, q'_E).\]
\end{IEEEproof}

\bigskip

\begin{theorem}
  \label{def:ioco_hiding}
Given a $\riolts$ $I$ and an $\iolts$ $S$ defined over the set $\OutputLabels$ of output labels, and  $\Sigma \subseteq \OutputLabels$, we have
$$
I \; \ioco \; S \rightarrow \fhide{I}{\Sigma} \; \ioco \; \fhide{S}{\Sigma}.
$$
\end{theorem}
\begin{IEEEproof}
Assume that $I \; \ioco\;S$ and $\Delta \in \straces{\fhide{S}{\Sigma}}$. 
Suppose 
\[\alpha \in \out{\fhide{I}{\Sigma} \;\after\; \Delta}{},\]
then we need to show that $\alpha \in \out{\fhide{S}{\Sigma} \;\after\; \Delta}{}$.

Let $\pi$ be a suspension trace in $I$ that becomes $\Delta$ after hiding and also leads to action $\alpha$
\[ \projection{\pi}{(\Labels_S\setminus \Sigma)\cup \{\delta\}} = \Delta \qquad \alpha\in \out{I \;\after\; \pi}{}. \]
Assume towards contradiction that $\pi \not\in \straces{S}$. 

Let $\pi'$ be the longest prefix of $\pi$ that is an s-trace in $S$. 
Let $\pi'\beta $ be the one action longer prefix of $\pi$.
Then $\beta$ cannot be an output action or $\delta$, because by Lemma \ref{lemma:outdelta}, $\pi'\beta$ would also be a prefix of $S$.
It follows that $\beta$ must be some input $i? \in \InputLabels_S$, so that
\[ \pi \in \straces{S} \qquad \pi i? \not\in \straces{S}. \]
This implies that there is a state $s$ in $\fhide{S}{\Sigma}$ after $\Delta'$ that cannot input $i?$
\[ s\in \fhide{S}{\Sigma} \;\after\; \Delta' \quad\text{s.t.}\quad s \not\xrightarrow{i?}.\]
Input actions are not hidden, so $\Delta$ can be written as:
\[ \Delta = \Delta'i?\Delta'' \quad\text{where}\quad \projection{\pi'}{(\Labels_A\setminus \Sigma)\cup \{\delta\}} = \Delta'.\]
From the assumption $\Delta \in \fhide{S}{\Sigma}$ it follows that there exists a state $s'$ reachable after $\Delta'$ that can accept $i?$
\[ s'\in \fhide{S}{\Sigma} \;\after\; \Delta' \quad\text{s.t.}\quad s' \xrightarrow{i?}.\]


Let $E$ be the friendly environment used in construction of $\fhide{S}{\Sigma}$.
Consider any state $(s',s_E)\in \fhide{S}{\Sigma}$, where $s_E$ belongs $E$. Environment does not distinguish between states reachable by the same traces, so $(s, s_E)$ would also be reachable in $\fhide{S}{\Sigma}$. This means that $s_E \not\xrightarrow{i}{}$, because otherwise $(s, s_E)$ would be an ambiguous state and $E$ would not be an environment. This implies that $\Delta'i? \not\in \straces{\fhide{S}{\Sigma}}$ which contradicts our assumption, therefore $\pi \in \straces{S}$.

Since $\pi$ is an an s-trace of $S$, then  by assumption $I \;\ioco\; S$ and by the fact $\alpha \in \out{I \;\after\; \pi}{}$ we get
\[\alpha\in \out{S \;\after\; \pi}{}\]
After hiding $\pi\alpha$ becomes s-trace $\Delta\alpha$ in $\fhide{S}{\Sigma}$, which proves the theorem.
\end{IEEEproof}




==> uioco.tex <==
\section{\textbf{Utraces}, $\uioco$ and Compositionality}
\label{sec:uioco}

In this section, we show that the $\uioco$ relation is not preserved under parallel composition and hiding. We first recall the 
definition of $\textbf{Utraces}$, as in~\cite{tretmans-comp}.

\begin{definition}
Given an $\iolts$ $A$, we define the set $\utraces{q}$, where $q \in Q$, as follows:
$$
\utraces{q} = \{ \sigma \in (\Labels\cup \{\delta\})^*~|~ q \xRightarrow{\sigma} \wedge (\not \exists q', \sigma_1\cdot \alpha \cdot \sigma_2 = 
\sigma~:~ \alpha \in \InputLabels \wedge q \xRightarrow{\sigma_1} q' \wedge q' \not \xRightarrow{\alpha} \}
$$
\end{definition}

The conformance relation $\uioco$ is defined as follows.

\begin{definition}
\label{def:uioco}
Given a $\riolts$ $I$ and an 
$\iolts$ $S$, we say that 
$I \; \uioco \; S$ iff
$$
\forall \sigma \in \utraces{S},\; \out{\qinit_{I} \; \after \; \sigma}{} \subseteq \out{\qinit_{S} \; \after \; \sigma}{}
$$
\end{definition}

\begin{theorem}
Given two composable $\riolts$ $I_{1}$ and $I_{2}$ and two composable $\iolts$ $S_{1}$ and $S_{2}$, we have
$$
\begin{array}{lcl}
I_{1} \; \uioco \; S_{1} \wedge I_{2} \; \uioco \; S_{2} &\not\rightarrow &(I_{1} \parallel I_{2}) \; \uioco \; (S_{1} \parallel S_{2}).
\end{array}
$$
\end{theorem}

\begin{IEEEproof}
In order to show that $\uioco$ is not preserved under parallel composition, we use the same example from~\cite{tretmans-comp} 
depicted in~Figure~\ref{fig:pc-uioco}, which 
was used to show non-compositionality of $\ioco$ under parallel composition. Since all the $\iolts$ ($S_1$, $S_2$, $I_1$, $I_2$, 
$S_1\parallel S_2$ and $I_1 \parallel I_2$), are deterministic and do not have $\tau$-transitions, there are no under-specified traces in 
any of the $\iolts$ and $\textbf{Utraces}$ coincide with the $\textbf{Straces}$. Hence, we have that $I_1 \; \uioco \; S_1$ and 
 $I_2 \; \uioco \; S_2$. Now consider the trace $x \in \utraces{S_1 \parallel S_2}$. We have that 
$\out{\qinit_{S_1 \parallel S_2} \; \after \; x}{} = \{ \delta \}$, 
while $\out{\qinit_{I_1 \parallel I_2} \; \after \; x}{} = \{ x \}$. It follows that $(I_{1} \parallel I_{2}) \; \not \uioco \; (S_{1} \parallel S_{2})$.
\end{IEEEproof}

\begin{figure}
\centering
\subfloat[][$S_1$]{\parbox[t]{2cm}{\centering \scalebox{0.6}{\begin{tikzpicture}[node distance=2cm,->,>=stealth',initial text=, thick]
\tikzstyle{state}=[circle, draw]
\tikzstyle{initstate}=[state,initial above]
\tikzstyle{transition}=[->,>=stealth']
\definecolor{currentcolor}{rgb}{0.000,0.000,0.000}
\node [initstate, draw=currentcolor] (state0) {1};
\node [state, draw=currentcolor, below of=state0] (state1) {2};
\path
	(state0) edge node[auto] {x?} (state1);
\end{tikzpicture}}}}%
\qquad
\subfloat[][$S_2$]{\parbox[t]{2cm}{\centering \scalebox{0.6}{\begin{tikzpicture}[node distance=2cm,->,>=stealth',initial text=, thick]
\tikzstyle{state}=[circle, draw]
\tikzstyle{initstate}=[state,initial above]
\tikzstyle{transition}=[->,>=stealth']
\definecolor{currentcolor}{rgb}{0.000,0.000,0.000}
\node [initstate, draw=currentcolor] (state0) {A};
\node [state, draw=currentcolor, below of=state0] (state1) {B};
\node [state, draw=currentcolor, below of=state1] (state2) {C};
\path
	(state0) edge node[auto] {x!} (state1)
	(state1) edge node[auto] {x!} (state2);
\end{tikzpicture}}}}%
\qquad
\subfloat[][$S_1 || S_2$]{\parbox[t]{2cm}{\centering \scalebox{0.6}{\begin{tikzpicture}[node distance=2cm,->,>=stealth',initial text=, thick]
\tikzstyle{state}=[circle, draw]
\tikzstyle{initstate}=[state,initial above]
\tikzstyle{transition}=[->,>=stealth']
\definecolor{currentcolor}{rgb}{0.000,0.000,0.000}
\node [initstate, draw=currentcolor] (state0) {I};
\node [state, draw=currentcolor, below of=state0] (state1) {II};
\path
	(state0) edge node[auto] {x!} (state1);
\end{tikzpicture}}}}%
\linebreak
\subfloat[][$I_1$]{\parbox[t]{2cm}{\centering \scalebox{0.6}{\begin{tikzpicture}[node distance=2cm,->,>=stealth',initial text=, thick]
\tikzstyle{state}=[circle, draw]
\tikzstyle{initstate}=[state,initial above]
\tikzstyle{transition}=[->,>=stealth']
\definecolor{currentcolor}{rgb}{0.000,0.000,0.000}
\node [initstate, draw=currentcolor] (state0) {1};
\node [state, draw=currentcolor, below of=state0] (state1) {2};
\path
	(state0) edge node[auto] {x?} (state1)
	(state1) edge [loop below] node [auto] {x?} (state1);
\end{tikzpicture}}}}%
\qquad
\subfloat[][$I_2$]{\parbox[t]{2cm}{\centering \scalebox{0.6}{\begin{tikzpicture}[node distance=2cm,->,>=stealth',initial text=, thick]
\tikzstyle{state}=[circle, draw]
\tikzstyle{initstate}=[state,initial above]
\tikzstyle{transition}=[->,>=stealth']
\definecolor{currentcolor}{rgb}{0.000,0.000,0.000}
\node [initstate, draw=currentcolor] (state0) {A};
\node [state, draw=currentcolor, below of=state0] (state1) {B};
\node [state, draw=currentcolor, below of=state1] (state2) {C};
\path
	(state0) edge node[auto] {x!} (state1)
	(state1) edge node[auto] {x!} (state2);
\end{tikzpicture}}}}%
\qquad
\subfloat[][$I_1||I_2$]{\parbox[t]{2cm}{\centering \scalebox{0.6}{\begin{tikzpicture}[node distance=2cm,->,>=stealth',initial text=, thick]
\tikzstyle{state}=[circle, draw]
\tikzstyle{initstate}=[state,initial above]
\tikzstyle{transition}=[->,>=stealth']
\definecolor{currentcolor}{rgb}{0.000,0.000,0.000}
\node [initstate, draw=currentcolor] (state0) {I};
\node [state, draw=currentcolor, below of=state0] (state1) {II};
\node [state, draw=currentcolor, below of=state1] (state2) {III};
\path
	(state0) edge node[auto] {x!} (state1)
	(state1) edge node[auto] {x!} (state2);
\end{tikzpicture}}}}%
\caption{Counter-example for preservation of $\uioco$ under parallel composition.}%
\label{fig:pc-uioco}%
\end{figure}

\begin{theorem}
Given a $\riolts$ $I$ and an $\iolts$ $S$, defined over the alphabet $\Labels$, and a subset $\Sigma \subseteq \OutputLabels$, we have
$$
\begin{array}{lcl}
I\ \uioco\ S &\not\rightarrow &\hide{I}{\Sigma}\ \uioco\ \hide{S}{\Sigma}.
\end{array}
$$
\end{theorem}

\begin{figure}
\centering
\subfloat[][Specification $S$]{\parbox[t]{4cm}{\centering \scalebox{0.6}{\begin{tikzpicture}[node distance=2cm,->,>=stealth',initial text=, thick]
\tikzstyle{state}=[circle, draw]
\tikzstyle{initstate}=[state,initial above]
\tikzstyle{transition}=[->,>=stealth']
\definecolor{currentcolor}{rgb}{0.000,0.000,0.000}
\node [initstate, draw=currentcolor] (state0) {1};
\node [state, draw=currentcolor, below of=state0] (state1) {2};
\node [state, draw=currentcolor, below of=state1] (state2) {3};

\path
	(state0) edge node[auto] {a!} (state1)
	(state1) edge node[auto] {i?} (state2)
			 edge[loop left] node [auto] {$\delta$} (state1)
	(state2) edge[loop below] node [auto] {$\delta$} (state2)
			 ;
\end{tikzpicture}}}}%
\qquad
\subfloat[][$S$ after hiding of a]{\parbox[t]{4cm}{\centering \scalebox{0.6}{\begin{tikzpicture}[node distance=2cm,->,>=stealth',initial text=, thick]
\tikzstyle{state}=[circle, draw]
\tikzstyle{initstate}=[state,initial above]
\tikzstyle{transition}=[->,>=stealth']
\definecolor{currentcolor}{rgb}{0.000,0.000,0.000}
\node [initstate, draw=currentcolor] (state0) {1};
\node [state, draw=currentcolor, below of=state0] (state1) {2};
\node [state, draw=currentcolor, below of=state1] (state2) {3};

\path
	(state0) edge node[auto] {$\tau$} (state1)
	(state1) edge node[auto] {i?} (state2)
			 edge[loop left] node [auto] {$\delta$} (state1)
	(state2) edge[loop below] node [auto] {$\delta$} (state2)
			 ;
\end{tikzpicture}}}}%
\linebreak
\subfloat[][Implementation $I$]{\scalebox{0.6}{\begin{tikzpicture}[node distance=2cm,->,>=stealth',initial text=, thick]
\tikzstyle{state}=[circle, draw]
\tikzstyle{initstate}=[state,initial above]
\tikzstyle{transition}=[->,>=stealth']
\definecolor{currentcolor}{rgb}{0.000,0.000,0.000}
\node [initstate, draw=currentcolor] (state0) {A};
\node [state, draw=currentcolor, below of=state0] (state1) {B};
\node [state, draw=currentcolor, below of=state1] (state2) {C};
\node [state, draw=currentcolor, right of=state0] (state3) {D};
\node [state, draw=currentcolor, right of=state3] (state4) {E};

\path
	(state0) edge node[auto] {a!} (state1)
			 edge node[auto] {i?} (state3)
	(state1) edge node[auto] {i?} (state2)
			 edge[loop left] node [auto] {$\delta$} (state1)
	(state2) edge[loop below] node [auto] {i?, $\delta$} (state2)
	(state3) edge node[auto] {b!} (state4)
			 edge [loop below] node[auto] {i?} (state3)
	(state4) edge[loop right] node [auto] {i?, $\delta$} (state4)
			 ;
\end{tikzpicture}}}%
\qquad
\subfloat[][$I$ after hiding of a]{\scalebox{0.6}{\begin{tikzpicture}[node distance=2cm,->,>=stealth',initial text=, thick]
\tikzstyle{state}=[circle, draw]
\tikzstyle{initstate}=[state,initial above]
\tikzstyle{transition}=[->,>=stealth']
\definecolor{currentcolor}{rgb}{0.000,0.000,0.000}
\node [initstate, draw=currentcolor] (state0) {A};
\node [state, draw=currentcolor, below of=state0] (state1) {B};
\node [state, draw=currentcolor, below of=state1] (state2) {C};
\node [state, draw=currentcolor, right of=state0] (state3) {D};
\node [state, draw=currentcolor, right of=state3] (state4) {E};

\path
	(state0) edge node[auto] {$\tau$} (state1)
			 edge node[auto] {i?} (state3)
	(state1) edge node[auto] {i?} (state2)
			 edge[loop left] node [auto] {$\delta$} (state1)
	(state2) edge[loop below] node [auto] {i?, $\delta$} (state2)
	(state3) edge node[auto] {b!} (state4)
			 edge [loop below] node[auto] {i?} (state3)
	(state4) edge[loop right] node [auto] {i?, $\delta$} (state4)
			 ;
\end{tikzpicture}}}
\caption{Counter-example for preservation of $\uioco$ under hiding.}%
\label{fig:h-uioco}%
\end{figure}

\begin{IEEEproof}
Consider the specification $S$ and the implementation $I$, depicted in Figures~\ref{fig:h-uioco}(a) and (c). It is clear that 
$I \; \uioco \; S$. Now consider $\hide{S}{\Sigma}$ and $\hide{I}{\Sigma}$ where $\Sigma = \{a\}$ (shown in 
 Figures~\ref{fig:h-uioco}(b) and (d)). We choose the trace $\sigma = i$ and show that it is in $\utraces{\hide{S}{\Sigma}}$. The only 
decomposition of $\sigma$ of the form $\sigma_1 \cdot \alpha \cdot \sigma_2$ such that $\alpha \in \InputLabels_{\hide{S}{\Sigma}}$ is 
$\epsilon \cdot i \cdot \epsilon$. Now, after reading the trace $\epsilon$, $\hide{S}{\Sigma}$ can be in either states $1$ or $2$. 
We have that both $1 \xRightarrow{i}  3$ and $2 \xRightarrow{i} 3$, hence $i \in \utraces{\hide{S}{\Sigma}}$. We have that 
$\out{\qinit_{\hide{S}{\Sigma}}{} \; \after \; i}{} = \{\delta\}$. On the other hand, $\out{\qinit_{\hide{I}{\Sigma}}{} \; \after \; i}{} = \{\delta, b\}$. 
It follows that $\hide{I}{\Sigma}\; \not \uioco \; \hide{S}{\Sigma}$.
\end{IEEEproof}


